PhysGraph: Physics-Based Integration Using Graph Neural Networks

Physics-based simulation of mesh based domains remains a challenging task. State-of-the-art techniques can produce realistic results but require expert knowledge. A major bottleneck in many approaches is the step of integrating a potential energy in order to compute velocities or displacements. Recently, learning based method for physics-based simulation have sparked interest with graph based approaches being a promising research direction. One of the challenges for these methods is to generate models that are mesh independent and generalize to different material properties. Moreover, the model should also be able to react to unforeseen external forces like ubiquitous collisions. Our contribution is based on a simple observation: evaluating forces is computationally relatively cheap for traditional simulation methods and can be computed in parallel in contrast to their integration. If we learn how a system reacts to forces in general, irrespective of their origin, we can learn an integrator that can predict state changes due to the total forces with high generalization power. We effectively factor out the physical model behind resulting forces by relying on an opaque force module. We demonstrate that this idea leads to a learnable module that can be trained on basic internal forces of small mesh patches and generalizes to different mesh typologies, resolutions, material parameters and unseen forces like collisions at inference time. Our proposed paradigm is general and can be used to model a variety of physical phenomena. We focus our exposition on the detail enhancement of coarse clothing geometry which has many applications including computer games, virtual reality and virtual try-on.

==> sections/figureOnlyPage.tex <==
\begin{figure*}[h]
  \centering
    \includegraphics[width=0.5\linewidth]{figures/fullPageResult3.png}
    \caption{We show several more examples of the cloth enhancement process using PhysGraph to demonstrate that our method scales to complicated multi-layer outfits. We demonstrate a tucked in shirt with belt and an outfit consisting of a hoodie, shirt and pants. Note how our model is capable of resolving collisions with small geometric features such as the belt loops and pockets.}
    \label{fig:fullPageResult}
\end{figure*}

==> sections/figureOnlyPage2.tex <==
\begin{figure*}[h]
  \centering
    \includegraphics[width=0.6\linewidth]{figures/temporalStability.png}
    \caption{We show several consecutive frames of an enhanced cloth sequence. Despite operating per frame, our method shows mostly temporally consistent results with the exception of collision heavy regions. Please refer to the supplemental video for the full result.}
    \label{fig:tshirtSequence}
\end{figure*}

==> sections/method-overview.tex <==
Our key contribution is the introduction of a learned module capable of integrating forces directly to the nodal positions of the graph while remaining agnostic to the origin of said forces. Our work is centered around this \emph{update module} which works in conjunction with a \emph{force module} which implements the appropriate potentials depending on the physical phenomenon being modeled. Given these complementary responsibilities of the modules, our method provides enormous flexibility to the system being modeled. The method is topology invariant since the forces are accumulated at the nodal level and, the update module is agnostic of the force generation process, allowing it to generalize to different types of potentials. 


An overview of the method is shown in Figure~\ref{fig:teaser}. \todo{check Fig ref}

%\PH{idea: framing the method as a multi-grid approach with basic smoothing and neural relaxation}. 

%\OH{Emphasize that our architectural paradigm is different than MeshGraphNet. The heart of the architecture is the physical force module that allows us to generalize to different forces unlike their architecture that once models the physical interaction cannot generalize to different systems where the forces are different.}


==> sections/method_old.tex <==
\section{Method}
\PH{Working on this section right now (offline). I will add the text tomorrow.}
Our key contribution is the introduction of a learned module capable of integrating forces directly to position updates of the nodal positions of the graph while remaining agnostic to the origin of these forces. Our work is centered around this \emph{integration module} which works in conjunction with a \emph{force module} which implements the appropriate potentials depending on the physical phenomenon being modeled. Given these complementary responsibilities of the modules, our method provides enormous flexibility to the system being modeled. The method is topology invariant since the forces are accumulated at the nodal level and, the integration module is agnostic to the force generation process, allowing it to generalize to different types of potentials even after the network is trained. 


An overview of the method is shown in Figure~\ref{fig:teaser}. \todo{check Fig ref}

\subsection{Graph-Based Physics Integration}

Our method operates on a physical system defined on a graph $G=(\textbf{V}, \textbf{E})$ with graph nodes $\textbf{V}$ and connections $\textbf{E}$.
\todo{can we generalize to a  more general domain other than graphs? The idea of the force module \& trajectory update policy is independent of the domain on which the system is defined}.%EL: IMO graphs are already a very general domain.
The system is specified as a general coordinate signal $\textbf{X} \in \mathcal{F}_G = \{f : \textbf{V} \rightarrow \mathbb{R}^d\}$ \PH{my personal preference: if we only work with a discrete graph domain, keep things more explicit $\mathbf{X} \in \mathbb R^{n \times d}$}, defined on the graph nodes $\textbf{V}$, and a potential function $\Phi : \mathcal{F}_G \rightarrow \mathbb{R}$ that describes the physical potential for every configuration of the graph coordinates. Our method aims to output the coordinate signal in the equilibrium state $\textbf{X}^* = \operatorname*{argmin}_{\textbf{X} \in \mathcal{F}_{G} , |\textbf{X} - \hat{\textbf{X}}| < r} \Phi(\text{high-resolution})$, that lies close within some radius $r$ as defined in the Hilbert space of the graph nodes' signals $\mathcal{F}_{G}$, to $\hat{\textbf{X}}$, given an input state.

Our approach learns a neural relaxation function $R : \mathcal{F}_{G} \rightarrow \mathcal{F}_{G}$ that takes the input signal $\hat{\textbf{X}}$ in combination with a provided potential function $\Phi$, and generates the equilibrium coordinates $\textbf{X}^*=R(\hat{\textbf{X}})$ of the physical system. We train the relaxation function by providing different physical systems at the training phase as an unsupervised loss term and let the neural model optimize the potential $\Phi$.

The function that updates the input coordinates to an equilibrium state, can be thought of as a sequence of $N$ recurring operations of a base function $f(\cdot)$. Namely, we decompose the relaxation function into the following form $R = f \circ f \circ ... \circ f$ where $f : \mathcal{F}_{G} \rightarrow \mathcal{F}_{G}$ generates an intermediate state with each application. The resulting intermediate states, $\{\textbf{X}_k\}_{k=0}^{k=N}$ form a trajectory in Hilbert space connecting the input state $\textbf{X}_0=\hat{\textbf{X}}$ with the output equilibrium state $\textbf{X}_N=\textbf{X}^*$.

%We design a universal model that is able to generalize to a variety of physical systems, different than the ones observed during training. Our architecture generalizes to different graph structures, potentials, and coordinate signals. 
We leverage a graph neural network with a physics-based architecture. The recurrent function $f(\cdot)$ consists of two sub-modules; A physics-based force module and a trainable integration network, that receives the partial history of the state trajectory and outputs the next state, see Figure \ref{fig:recurrent-function}.

\begin{figure}[h]
\centering % used for centering Figure
\includegraphics[trim={0 0 0 3cm},clip, width=0.45 \textwidth]{figures/recurrent unit diagram.png}
\caption{The coordinate signal of the physical system $\textbf{X}_k$ is updated recurrently by the function $f$ consisting of a force and an integration module, that produces the next state $\textbf{X}_{k+1}=f(\textbf{X}_k)$. \todo{Highlight which parts of the pipeline are learned (integration module) which ones are analytical expression (force module)} \PH{short descriptions of $S_k$ and $D_k$ help parsing the figure.} \todo{change walker to integration module}}
\label{fig:recurrent-function}
\end{figure}

\subsection{Force Module}

We credit the generalizability of our method to  separation of the force formulation and integration. The force generation module outputs forces based on user-specified potentials given the current nodal configuration where forces are accumulated at the nodal level, enabling parallellization of the force computation. The conservative force potential $\Phi$, is responsible for the forces $\textbf{F}=-\nabla_\textbf{X}\Phi$ acting on the system. Different potentials can be used to model different physical phenomena.  

%In our framework, we have the capability of modeling various systems depending on the provided potentials. In contrast, a network that models this relation explicitly $\textbf{X}_k \rightarrow \textbf{F}_k \rightarrow \textbf{X}_{k+1}$ or implicitly $\textbf{X}_k \rightarrow \textbf{X}_{k+1}$ would be bound to overfit to the training data since the relation $\textbf{X}_k \rightarrow \textbf{F}_k$ is a specific characteristic of a physical system and the forces at play. In contrast, we learn the universal update rule with the force characteristics provided by the force module directly.

%On the other hand, having access to the force signal $\textbf{F}_k$ in every state $\textbf{X}_k$ (and optionally to higher order derivatives of the potential), a trajectory update policy to reach the equilibrium state could be devised that is universal. For example, the simplest trajectory update policy would be $\textbf{X}_{k+1} = \textbf{X}_k + \epsilon (\textbf{F}_k)$.%w\ZB{ sorry for the nit-picking, but adding location units to scalar times force could be changed. e.g. $\textbf{X}_{k+1} = \textbf{X}_k + \epsilon(\textbf{F}_k$})).

%\subsection{Graph-Based Force Integration Update Module}
\subsection{Integration Module}
\label{updateModule}

\todo{This section needs work}

The integration module is a learned trajectory-aware optimizer on the landscape defined by the physical potential provided by the force module. This integration module is a function that receives the system trajectory in state-space $\textbf{X}_k, \textbf{X}_{k-1}, ...$ and the exerted forces along this trajectory $\textbf{F}_k, \textbf{F}_{k-1}, ...$ and outputs the next state $\textbf{X}_{k+1}$. Let $\textbf{S}_k=(\textbf{X}_k, \textbf{F}_k, \textbf{X}_{k-1}, \textbf{F}_{k-1}, ...)$ be the sequence of system coordinates and forces signals. The integration module is a learned function $w_\theta : \textbf{X}_k, \textbf{F}_k, \textbf{S}_{k-1} \rightarrow \textbf{D}_k$, where $\theta$ are the learned parameters. The next state $\textbf{X}_{k+1}$ is updated by adding the displacement signal $\textbf{D}_k$ to the current state $\textbf{X}_{k+1} = \textbf{X}_k + \textbf{D}_k$.

Staring from the initial condition, these forces in turn determine the system state evolution towards equilibrium, $\textbf{X}_0 \rightarrow ... \rightarrow \textbf{X}^*$. 

When implementing the functional form of $w_\theta$, we wish to provide the module with the ability to make an update $\textbf{D}_k(v)$ to the node $v \in V$, based on additional information.
%than the values of the trajectory signals at that specific node, namely $S_k(v)=(X_k(v), F_k(v), X_{k-1}(v), F_{k-1}(v), ...)$. Instead, 
We devise a functional form that allows $\textbf{D}_k(v)$ to be predicted based on the trajectory signals sampled at an extended local neighborhood of $v$ \PH{could be more explicit}. Thus, local patterns in the trajectory signals can be learned, allowing a better update policy compared to node-wise based policy. Using a local update-rule makes the scatter module function highly parallelizable. This feature can be exploited to accelerate its computation time. %\todo{In the analysis section it would be nice to show some force patterns characteristic to different types of forces, and the resulting displacement signals.} \todo{Should we mention performance related things or not since we do not focus on that?}
Our choice for local updates and the requirement to generalize different graph topologies leads us to choose a message-passing network \cite{pfaff2020learning} as the architecture of the update rule, which generally admits those criteria.


For the integration module, we use a similar architecture as MeshGraphNet \cite{pfaff2020learning}, with the exception that we do not require world-edges since the spatial proximity between the nodes in world space is implicitly represented by the collision force signal. Let $\textbf{S}_k=\left(\textbf{X}_k, \textbf{F}_k, \textbf{X}_{k-1}, \textbf{F}_{k-1}, ..., \textbf{X}_0, \textbf{F}_0\right)$ be the sequence of system coordinates and forces signals after the k-recurrent block, we define the input node signals to the integration module in the (k+1)-recurrent block as the truncated sequence of first order differences of the coordinates, and the forces \PH{define vertex and edge signal first.}.
\begin{equation}
%\begin{split}
%    n_0 = (&\textbf{X}_k - \textbf{X}_{k-1}, \textbf{X}_{k-1} - \textbf{X}_{k-2}, ..., \textbf{X}_{k-H} - \textbf{X}_{k-H-1}, \\
%    &\textbf{F}_k, \textbf{F}_{k-1}, ..., \textbf{F}_{k-H})
%\end{split}
    n_0 = \left(\textbf{X}_k - \textbf{X}_{k-1}, ..., \textbf{X}_{k-H} - \textbf{X}_{k-H-1}, \textbf{F}_k, \textbf{F}_{k-1}, ..., \textbf{F}_{k-H}\right)
\end{equation}
treating the signals as constants for non-positive indices, namely: $\textbf{X}_i = \textbf{X}_0, \textbf{F}_i = \textbf{F}_0, \forall i< 0$. With this definition, the input node signal is invariant to the translation of the physical system.
The edge input signals are defined similarly as MeshGraphNet, where $\textbf{X}(\cdot)$ and $\textbf{u}(\cdot)$ are the world and mesh coordinates, respectively. This definition is also translation invariant.
\begin{equation}
\begin{split}
    (e_0)_{v_i,v_j} = ( &X_k(v_i) - X_k(v_j), | X_k(v_i) - X_k(v_j) |, \\
    & u_k(v_i) - u_k(v_j), | u_k(v_i) - u_k(v_j) | ) 
\end{split}
\end{equation}
Then input node and edge signals are then passed into the same Encoder-Processor-Decoder architecture as in MeshGraphNet, producing an output node-signal with feature dimension = 3, which is interpreted as the displacement $D_k$. \todo{The architecture parameters we use are available at the supplementary material.}

==> sections/neural-upsampling.tex <==
%\PH{Maybe I am missing the point here but isn't this what we are doing in any case? What is different?}

%One of the applications of physics-based integration is a high-resolution simulation of physical systems with conservative energies. A physical system could be simulated fast using a classical physical simulator, over a coarse graph $\tilde{G} = (\tilde{\textbf{V}}, \tilde{\textbf{E}})$, producing a coarse simulation signal $\tilde{\textbf{X}} \in \mathcal{\textbf{F}}_{\tilde{G}} = \{f : \tilde{\textbf{V}} \rightarrow \mathbb{R}^d\}$. Then, a subdivision scheme is applied to the coarse graph, obtaining a high-resolution graph $G = (\textbf{V}, \textbf{E})$, on which the high-resolution simulation signal would be defined. To get the high-resolution simulation signal $\textbf{X} \in \mathcal{F}_{G} = \{f : \textbf{V} \rightarrow \mathbb{R}^d\}$, we perform physics-based integration with the model described in the previous section. Using $\hat{\textbf{X}}$, the linear interpolation of the coarse coordinate signal $\tilde{\textbf{X}}$, as the input state $\textbf{X}_0=\hat{\textbf{X}}$. The potential function $\Phi$ and the \emph{Oracle}: $\textbf{F}=-\nabla_\textbf{X}\Phi$ should be defined for the system of interest, based on the specific quasi-static model that accounts for the detail generation. In the next section, we show how we apply this formulation to perform upsampling of cloth simulation.
